An effectful object calculus

We show how to smoothly incorporate in the object-oriented paradigm constructs to raise, compose, and handle effects in an arbitrary monad. The underlying pure calculus is meant to be a representative of the last generation of OO languages, and the effectful extension is manageable enough for ordinary programmers; notably, constructs to raise effects are just special methods. We equip the calculus with an expressive type-and-effect system, which, again by relying on standard features such as inheritance and generic types, allows a simple form of effect polymorphism. The soundness of the type-and-effect system is expressed and proved by a recently introduced technique, where the semantics is formalized by a one-step reduction relation from language expressions into monadic ones, so that it is enough to prove progress and subject reduction properties on this relation.

==> conf-bib-macros.tex <==

\newcommand{\APLAS}[2]{Proceedings of the #1 Asian Symposium on Programming Languages and Systems, {APLAS} #2} 

\newcommand{\CMCS}[2]{Proceedings of the #1 Workshop on Coalgebraic Methods in Computer Science, {CMCS} #2} 


\newcommand{\ECOOP}[2]{#1 European Conference on Object-Oriented Programming, {ECOOP} #2}
\newcommand{\ESOP}[2]{Programming Languages and Systems - #1 European Symposium on Programming, {ESOP} #2} 
\newcommand{\FOSSACS}[2]{Foundations of Software Science and Computation Structures, #1 International Conference, {FoSSaCS} #2}
\newcommand{\FSCD}[2]{#1 International Conference on Formal Structures for Computation and Deduction, {FSCD} 2017} 
\newcommand{\ICFP}[2]{#1 {ACM} {SIGPLAN} International Conference on Functional Programming, {ICFP} #2} 
\newcommand{\LICS}[2]{Proceedings of the #1 Annual {ACM/IEEE} Symposium on Logic in Computer Science, {LICS} #2}
\newcommand{\MFPS}[2]{The #1 Conference on Mathematical Foundations of Programming Semantics, {MFPS} #2} 
\newcommand{\POPL}[2]{Proceedings of the #1 {ACM/SIGPLAN} Symposium on Principles of Programming Languages, {POPL} #2} 
\newcommand{\OOPSLA}[2]{Proceedings of the #1 {ACM} International Conference on Object-Oriented Programming: Systems, Languages and Applications, {OOPSLA} #2}



